MDP: A Generalized Framework for Text-Guided Image Editing by Manipulating the Diffusion Path

Image generation using diffusion can be controlled in multiple ways. In this paper, we systematically analyze the equations of modern generative diffusion networks to propose a framework, called MDP, that explains the design space of suitable manipulations. We identify 5 different manipulations, including intermediate latent, conditional embedding, cross attention maps, guidance, and predicted noise. We analyze the corresponding parameters of these manipulations and the manipulation schedule. We show that some previous editing methods fit nicely into our framework. Particularly, we identified one specific configuration as a new type of control by manipulating the predicted noise, which can perform higher-quality edits than previous work for a variety of local and global edits.

==> figures/tex/diffusion.tex <==
\resizebox{\linewidth}{!}{%
    \begin{tikzpicture}[->,>=stealth',auto,
      thick,
      data node/.style={rectangle,draw,font=\sffamily\LARGE\bfseries, minimum width=1.7cm, minimum height=1.7cm},
      func node/.style={circle,draw,font=\sffamily\LARGE\bfseries, minimum width=2cm, minimum height=1cm},
      ] 
        \LARGE
        \pgfdeclarelayer{background}
        \pgfsetlayers{background, main}
        
        \node[data node, draw=aabbcc!80, fill=aabbcc!10] (x) {$\mathbf{x}_{T}$};
        \node[func node, above=0.7cm of x, draw=aabbee!80, fill=aabbee!10] (unet){$\boldsymbol\epsilon_\theta$};
        \draw[->] (x) -- (unet);
        \node[func node, right=0.7cm of x] (ddim) {$\mathrm{DDIM}$};
        \node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim |- unet) (n) {$\boldsymbol\epsilon_{T}$};
        \draw[->] (unet) -- (n);
        \draw[->] (n) -- (ddim);
        \draw[->] (x) -- (ddim);
        % \draw[->] (ddim-t) -- +(0:2);
        % \draw[<-] (x-t) -- +(180:2);
        \node[data node, above=0.7cm of unet, draw=aaddee!80, fill=aaddee!10] (c) {$\mathbf{c}$};
        \draw[->] (c) -- (unet);
        
        \begin{pgfonlayer}{background}
        \node [fit=(x)(unet)(n)(ddim)(c), label={above:Step $T$}, fill=aaddff!10] {}; 
        \end{pgfonlayer}

        \node[data node, right=0.7cm of ddim, draw=aaccff!80, fill=aaccff!10] (x-t-1) {$\mathbf{x}_{T-1}$};
        \node[func node, above=0.7cm of x-t-1, draw=aabbee!80, fill=aabbee!10] (unet-t-1){$\boldsymbol\epsilon_\theta$};
        \draw[->] (x-t-1) -- (unet-t-1);
        \node[func node, right=0.7cm of x-t-1] (ddim-t-1) {$\mathrm{DDIM}$};
        \node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-t-1 |- unet-t-1) (n-t-1) {$\boldsymbol\epsilon_{T-1}$};
        \draw[->] (unet-t-1) -- (n-t-1);
        \draw[->] (n-t-1) -- (ddim-t-1);
        \draw[->] (x-t-1) -- (ddim-t-1);
        % \draw[->] (ddim-t) -- +(0:2);
        % \draw[<-] (x-t) -- +(180:2);
        \node[data node, above=0.7cm of unet-t-1, draw=aaddee!80, fill=aaddee!10] (c-t-1) {$\mathbf{c}$};
        \draw[->] (c-t-1) -- (unet-t-1);
        

        \begin{pgfonlayer}{background}
        \node [fit=(x-t-1)(unet-t-1)(n-t-1)(ddim-t-1)(c-t-1), label={above:Step $T-1$}, fill=aaddff!10] {}; 
        \end{pgfonlayer}
        
        \draw[->] (ddim) -- (x-t-1);

        \node[right=0.7cm of ddim-t-1] (dots) {$\dots$};
        \draw[->] (ddim-t-1) -- (dots);
        
        \node[data node, right=0.7cm of dots, draw=aaccff!80, fill=aaccff!10] (x-t) {$\mathbf{x}_{t}$};
        \node[func node, above=0.7cm of x-t, draw=aabbee!80, fill=aabbee!10] (unet-t){$\boldsymbol\epsilon_\theta$};
        \draw[->] (x-t) -- (unet-t);
        \node[func node, right=0.7cm of x-t] (ddim-t) {$\mathrm{DDIM}$};
        \node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-t |- unet-t) (n-t) {$\boldsymbol\epsilon_{t}$};
        \draw[->] (unet-t) -- (n-t);
        \draw[->] (n-t) -- (ddim-t);
        \draw[->] (x-t) -- (ddim-t);
        % \draw[->] (ddim-t) -- +(0:2);
        % \draw[<-] (x-t) -- +(180:2);
        \node[data node, above=0.7cm of unet-t, draw=aaddee!80, fill=aaddee!10] (c-t) {$\mathbf{c}$};
        \draw[->] (c-t) -- (unet-t);
        

        \begin{pgfonlayer}{background}
        \node [fit=(x-t)(unet-t)(n-t)(ddim-t)(c-t), label={above:Step $t$}, fill=aaddff!10] {}; 
        \end{pgfonlayer}

        \draw[->] (dots) -- (x-t);

        \node[right=0.7cm of ddim-t] (dots2) {$\dots$};
        \draw[->] (ddim-t) -- (dots2);

        \node[data node, right=0.7cm of dots2, draw=aaccff!80, fill=aaccff!10] (x-1) {$\mathbf{x}_{1}$};
        \node[func node, above=0.7cm of x-1, draw=aabbee!80, fill=aabbee!10] (unet-1){$\boldsymbol\epsilon_\theta$};
        \draw[->] (x-1) -- (unet-1);
        \node[func node, right=0.7cm of x-1] (ddim-1) {$\mathrm{DDIM}$};
        \node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-1 |- unet-1) (n-1) {$\boldsymbol\epsilon_{1}$};
        \draw[->] (unet-1) -- (n-1);
        \draw[->] (n-1) -- (ddim-1);
        \draw[->] (x-1) -- (ddim-1);
        % \draw[->] (ddim-t) -- +(0:2);
        % \draw[<-] (x-t) -- +(180:2);
        \node[data node, above=0.7cm of unet-1, draw=aaddee!80, fill=aaddee!10] (c-1) {$\mathbf{c}$};
        \draw[->] (c-1) -- (unet-1);

        \begin{pgfonlayer}{background}
        \node [fit=(x-1)(unet-1)(n-1)(ddim-1)(c-1), label={above:Step $1$}, fill=aaddff!10] {}; 
        \end{pgfonlayer}
        
        \draw[->] (dots2) -- (x-1);
        
        \node[data node, right=0.7cm of ddim-1] (x-0) {$\mathbf{x}_{0}$};

        \draw[->] (ddim-1) -- (x-0);
    \end{tikzpicture}
}

==> figures/tex/pipeline.tex <==
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
->,>=stealth',auto,
      % thick,
      data node/.style={rectangle,draw,font=\sffamily\LARGE, minimum width=1.2cm, minimum height=1.2cm},
      func node/.style={circle,draw,font=\sffamily\LARGE, minimum width=1.5cm, minimum height=0.4cm},
]
\LARGE
\pgfdeclarelayer{background}
\pgfdeclarelayer{bbackground}
\pgfsetlayers{bbackground, background, main}
        
\node[data node, draw=aabbcc!80, fill=aabbcc!10, label={[name=x-name]below: $\mathbf{x}_{T}\phantom{^{(A)}}$}] (x) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xa/50.jpg}
};

\node[func node, right=0.4cm of x] (ddim) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x] (unet) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim |- unet) (n) {$\textcolor{A}{\boldsymbol\epsilon_{T}^{(A)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet] (c) {$\textcolor{A}{\mathbf{c}^{(A)}}$};

\draw[->] (x) -- (ddim);
\draw[->] (unet) -- (n);
\draw[->] (x) -- (unet);
\draw[->] (n) -- (ddim);
\draw[->] (c) -- (unet);

\begin{pgfonlayer}{background}
\node [fit=(x)(unet)(n)(ddim)(c), label={above:Step $T$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

\node[right=0.4cm of ddim] (dots3) {$\dots$};
\draw[->] (ddim) -- (dots3);

\node[data node, draw=aaccff!80, fill=aaccff!10, right=0.4cm of dots3, label={below: $\textcolor{A}{\mathbf{x}_{t_{\text{max}}}^{(A)}}$}] (x-t-1) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xa/30.jpg}
};

\node[func node, right=0.4cm of x-t-1] (ddim-t-1) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-t-1] (unet-t-1) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-t-1 |- unet-t-1) (n-t-1) {$\textcolor{A}{\boldsymbol\epsilon_{t_{\text{max}}}^{(A)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet-t-1] (c-t-1) {$\textcolor{A}{\mathbf{c}^{(A)}}$};

\draw[->] (x-t-1) -- (ddim-t-1);
\draw[->] (unet-t-1) -- (n-t-1);
\draw[->] (x-t-1) -- (unet-t-1);
\draw[->] (n-t-1) -- (ddim-t-1);
\draw[->] (c-t-1) -- (unet-t-1);

\begin{pgfonlayer}{background}
\node [fit=(x-t-1)(unet-t-1)(n-t-1)(ddim-t-1)(c-t-1), label={above:Step $t_{\text{max}}$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

% \draw[->] (ddim) -- (x-t-1);
\draw[->] (dots3) -- (x-t-1);



\node[right=0.4cm of ddim-t-1] (dots) {$\dots$};
\draw[->] (ddim-t-1) -- (dots);
        
\node[data node, draw=aaccff!80, fill=aaccff!10, right=0.4cm of dots, label={below: $\textcolor{A}{\mathbf{x}_{t_{\text{min}}}^{(A)}}$}] (x-t) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xa/20.jpg}
};

\node[func node, right=0.4cm of x-t] (ddim-t) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-t] (unet-t) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-t |- unet-t) (n-t) {$\textcolor{A}{\boldsymbol\epsilon_{t_{\text{min}}}^{(A)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet-t] (c-t) {$\textcolor{A}{\mathbf{c}^{(A)}}$};

\draw[->] (x-t) -- (ddim-t);
\draw[->] (unet-t) -- (n-t);
\draw[->] (x-t) -- (unet-t);
\draw[->] (n-t) -- (ddim-t);
\draw[->] (c-t) -- (unet-t);

\begin{pgfonlayer}{background}
\node [fit=(x-t)(unet-t)(n-t)(ddim-t)(c-t), label={above:Step $t_{\text{min}}$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

\draw[->] (dots) -- (x-t);


\node[right=0.4cm of ddim-t] (dots2) {$\dots$};
\draw[->] (ddim-t) -- (dots2);
        
\node[data node, draw=aaccff!80, fill=aaccff!10, right=0.4cm of dots2, label={below: $\textcolor{A}{\mathbf{x}_{1}^{(A)}}$}] (x-1) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xa/10.jpg}
};

\node[func node, right=0.4cm of x-1] (ddim-1) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-1] (unet-1) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-1 |- unet-1) (n-1) {$\textcolor{A}{\boldsymbol\epsilon_{1}^{(A)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet-1] (c-1) {$\textcolor{A}{\mathbf{c}^{(A)}}$};

\draw[->] (x-1) -- (ddim-1);
\draw[->] (unet-1) -- (n-1);
\draw[->] (x-1) -- (unet-1);
\draw[->] (n-1) -- (ddim-1);
\draw[->] (c-1) -- (unet-1);

\begin{pgfonlayer}{background}
\node [fit=(x-1)(unet-1)(n-1)(ddim-1)(c-1), label={[name=step-name]above:Step $1$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

\draw[->] (dots2) -- (x-1);

\node[data node, draw, right=0.4cm of ddim-1, label={below: $\textcolor{A}{\mathbf{x}_{0}^{(A)}}$}] (x-0) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xa/1.jpg}
};

\draw[->] (ddim-1) -- (x-0);

\begin{pgfonlayer}{bbackground}
\node [fit=(x)(unet)(n)(ddim)(c)(x-0)(x-name)(step-name), fill=aaddgg!10, label={right: \rotatebox{-90}{%Generated given condition 
$\textcolor{A}{\mathbf{c}^{(A)}}$}}] {}; 
\end{pgfonlayer}

%%%%%
\node[data node, draw=aabbcc!80, fill=aabbcc!10, label={[name=x-name]below: $\mathbf{x}_{T}\phantom{^{(B)}}$}, below=7cm of x] (x) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xb/50.jpg}
};

\node[func node, right=0.4cm of x] (ddim) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x] (unet) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim |- unet) (n) {$\textcolor{B}{\boldsymbol\epsilon_{T}^{(B)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet] (c) {$\textcolor{B}{\mathbf{c}^{(B)}}$};

\draw[->] (x) -- (ddim);
\draw[->] (unet) -- (n);
\draw[->] (x) -- (unet);
\draw[->] (n) -- (ddim);
\draw[->] (c) -- (unet);


\begin{pgfonlayer}{background}
\node [fit=(x)(unet)(n)(ddim)(c), label={above:Step $T$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

\node[right=0.4cm of ddim] (dots3) {$\dots$};
\draw[->] (ddim) -- (dots3);

\node[data node, draw=aaccff!80, fill=aaccff!10, right=0.4cm of dots3, label={below: $\textcolor{B}{\mathbf{x}_{t_{\text{max}}}^{(B)}}$}] (x-t-1) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/epsilon/30.jpg}
};

\node[func node, right=0.4cm of x-t-1] (ddim-t-1) {DDIM};

\phantom{\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-t-1] (unet-t-1) {$\boldsymbol\epsilon_\theta$};}

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-t-1 |- unet-t-1) (n-t-1-copy) {$\textcolor{A}{\boldsymbol\epsilon_{t_{\text{max}}}^{(A)}}$};

\phantom{\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet-t-1] (c-t-1) {$\textcolor{B}{\mathbf{c}^{(B)}}$};}

\draw[->] (x-t-1) -- (ddim-t-1);
% \draw[->] (unet-t-1) -- (n-t-1);
% \draw[->] (x-t-1) -- (unet-t-1);
\draw[->] (n-t-1-copy) -- (ddim-t-1);
% \draw[->] (c-t-1) -- (unet-t-1);


\draw[dashed, ->] ([yshift=0pt]n-t-1.south east) to[bend left] node[above, midway, sloped] {Copy} ([yshift=0pt]n-t-1-copy.north east) ;

\begin{pgfonlayer}{background}
\node [fit=(x-t-1)(unet-t-1)(n-t-1-copy)(ddim-t-1)(c-t-1), label={above:Step $t_{\text{max}}$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

% \draw[->] (ddim) -- (x-t-1);
\draw[->] (dots3) -- (x-t-1);


\node[right=0.4cm of ddim-t-1] (dots) {$\dots$};
\draw[->] (ddim-t-1) -- (dots);
        
\node[data node, draw=aaccff!80, fill=aaccff!10, right=0.4cm of dots, label={below: $\textcolor{star}{\mathbf{x}_{t_{\text{min}}}^{(\star)}}$}] (x-t) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/epsilon/20.jpg}
};

\node[func node, right=0.4cm of x-t] (ddim-t) {DDIM};

\phantom{\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-t] (unet-t) {$\boldsymbol\epsilon_\theta$};}

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-t |- unet-t) (n-t-copy) {$\textcolor{A}{\boldsymbol\epsilon_{t_{\text{min}}}^{(A)}}$};

\phantom{\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet-t] (c-t) {$\textcolor{B}{\mathbf{c}^{(B)}}$};}

\draw[->] (x-t) -- (ddim-t);
% \draw[->] (unet-t) -- (n-t);
% \draw[->] (x-t) -- (unet-t);
\draw[->] (n-t-copy) -- (ddim-t);
% \draw[->] (c-t) -- (unet-t);

\draw[dashed, ->] ([yshift=0pt]n-t.south east) to[bend left] node[above, midway, sloped] {Copy} ([yshift=0pt]n-t-copy.north east) ;

\begin{pgfonlayer}{background}
\node [fit=(x-t)(unet-t)(n-t-copy)(ddim-t)(c-t), label={above:Step $t_{\text{min}}$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

\draw[->] (dots) -- (x-t);


\node[right=0.4cm of ddim-t] (dots2) {$\dots$};
\draw[->] (ddim-t) -- (dots2);
        
\node[data node, draw=aaccff!80, fill=aaccff!10, right=0.4cm of dots2, label={below: $\textcolor{star}{\mathbf{x}_{1}^{(\star)}}$}] (x-1) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/epsilon/10.jpg}
};

\node[func node, right=0.4cm of x-1] (ddim-1) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-1] (unet-1) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-1 |- unet-1) (n-1) {$\textcolor{star}{\boldsymbol\epsilon_{1}^{(\star)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet-1] (c-1) {$\textcolor{B}{\mathbf{c}^{(B)}}$};

\draw[->] (x-1) -- (ddim-1);
\draw[->] (unet-1) -- (n-1);
\draw[->] (x-1) -- (unet-1);
\draw[->] (n-1) -- (ddim-1);
\draw[->] (c-1) -- (unet-1);

\begin{pgfonlayer}{background}
\node [fit=(x-1)(unet-1)(n-1)(ddim-1)(c-1), label={[name=step-name]above:Step $1$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

\draw[->] (dots2) -- (x-1);

\node[data node, draw, right=0.4cm of ddim-1, label={below: $\textcolor{star}{\mathbf{x}_{0}^{(\star)}}$}] (x-0) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/epsilon/1.jpg}
};

\draw[->] (ddim-1) -- (x-0);

\begin{pgfonlayer}{bbackground}
\node [fit=(x)(unet)(n)(ddim)(c)(x-0)(x-name)(step-name), fill=aaddgg!10, label={right: \rotatebox{-90}{Edited}}] {}; 
\end{pgfonlayer}


%%%%%
\node[data node, draw=aabbcc!80, fill=aabbcc!10, label={[name=x-name]below: $\mathbf{x}_{T}\phantom{^{(A)}}$}, below=7cm of x] (x-copy) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xb/50.jpg}
};

% \draw[dashed, <-] ([yshift=0pt]x.south west) to[bend right] node[above, midway, sloped] {Copy} ([yshift=0pt]x-copy.north west);

\node[func node, right=0.4cm of x-copy] (ddim) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-copy] (unet) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim |- unet) (n) {$\textcolor{B}{\boldsymbol\epsilon_{T}^{(B)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet] (c) {$\textcolor{B}{\mathbf{c}^{(B)}}$};

\draw[->] (x-copy) -- (ddim);
\draw[->] (unet) -- (n);
\draw[->] (x-copy) -- (unet);
\draw[->] (n) -- (ddim);
\draw[->] (c) -- (unet);

\begin{pgfonlayer}{background}
\node [fit=(x-copy)(unet)(n)(ddim)(c), label={above:Step $T$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

\node[right=0.4cm of ddim] (dots3) {$\dots$};
\draw[->] (ddim) -- (dots3);

\node[data node, draw=aaccff!80, fill=aaccff!10, right=0.4cm of dots3, label={below: $\textcolor{B}{\mathbf{x}_{t_{\text{max}}}^{(B)}}$}] (x-t-1-copy) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xb/30.jpg}
};

% \draw[dashed, <-] ([yshift=0pt]x-t-1.south west) to[bend right] node[above, midway, sloped] {Copy} ([yshift=0pt]x-t-1-copy.north west);

\node[func node, right=0.4cm of x-t-1-copy] (ddim-t-1) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-t-1-copy] (unet-t-1) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-t-1 |- unet-t-1) (n-t-1) {$\textcolor{B}{\boldsymbol\epsilon_{t_{\text{max}}}^{(B)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet-t-1] (c-t-1) {$\textcolor{B}{\mathbf{c}^{(B)}}$};

\draw[->] (x-t-1-copy) -- (ddim-t-1);
\draw[->] (unet-t-1) -- (n-t-1);
\draw[->] (x-t-1-copy) -- (unet-t-1);
\draw[->] (n-t-1) -- (ddim-t-1);
\draw[->] (c-t-1) -- (unet-t-1);

% \draw[dashed, ->] ([yshift=0pt]n-t-1.south east) to[bend left] node[above, midway, sloped] {Copy} ([yshift=0pt]n-t-1-copy.north east) ;

\begin{pgfonlayer}{background}
\node [fit=(x-t-1-copy)(unet-t-1)(n-t-1)(ddim-t-1)(c-t-1), label={above:Step $t_{\text{max}}$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

% \draw[->] (ddim) -- (x-t-1);
\draw[->] (dots3) -- (x-t-1-copy);


\node[right=0.4cm of ddim-t-1] (dots) {$\dots$};
\draw[->] (ddim-t-1) -- (dots);
        
\node[data node, draw=aaccff!80, fill=aaccff!10, right=0.4cm of dots, label={below: $\textcolor{B}{\mathbf{x}_{t_{\text{min}}}^{(B)}}$}] (x-t) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xb/20.jpg}
};

\node[func node, right=0.4cm of x-t] (ddim-t) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-t] (unet-t) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-t |- unet-t) (n-t) {$\textcolor{B}{\boldsymbol\epsilon_{t_{\text{min}}}^{(B)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet-t] (c-t) {$\textcolor{B}{\mathbf{c}^{(B)}}$};

\draw[->] (x-t) -- (ddim-t);
\draw[->] (unet-t) -- (n-t);
\draw[->] (x-t) -- (unet-t);
\draw[->] (n-t) -- (ddim-t);
\draw[->] (c-t) -- (unet-t);

% \draw[dashed, ->] ([yshift=0pt]n-t.south east) to[bend left] node[above, midway, sloped] {Copy} ([yshift=0pt]n-t-copy.north east) ;

\begin{pgfonlayer}{background}
\node [fit=(x-t)(unet-t)(n-t)(ddim-t)(c-t), label={above:Step $t_{\text{min}}$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

\draw[->] (dots) -- (x-t);


\node[right=0.4cm of ddim-t] (dots2) {$\dots$};
\draw[->] (ddim-t) -- (dots2);
        
\node[data node, draw=aaccff!80, fill=aaccff!10, right=0.4cm of dots2, label={below: $\textcolor{B}{\mathbf{x}_{1}^{(B)}}$}] (x-1) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xb/10.jpg}
};

\node[func node, right=0.4cm of x-1] (ddim-1) {DDIM};

\node[func node, draw=aabbee!80, fill=aabbee!10, above=0.4cm of x-1] (unet-1) {$\boldsymbol\epsilon_\theta$};

\node[data node, draw=aabbff!80, fill=aabbff!10] at (ddim-1 |- unet-1) (n-1) {$\textcolor{B}{\boldsymbol\epsilon_{1}^{(B)}}$};

\node[data node, draw=aaddee!80, fill=aaddee!10, above=0.4cm of unet-1] (c-1) {$\textcolor{B}{\mathbf{c}^{(B)}}$};

\draw[->] (x-1) -- (ddim-1);
\draw[->] (unet-1) -- (n-1);
\draw[->] (x-1) -- (unet-1);
\draw[->] (n-1) -- (ddim-1);
\draw[->] (c-1) -- (unet-1);

\begin{pgfonlayer}{background}
\node [fit=(x-1)(unet-1)(n-1)(ddim-1)(c-1), label={[name=step-name]above:Step $1$}, fill=aaddff!10] {}; 
\end{pgfonlayer}

\draw[->] (dots2) -- (x-1);

\node[data node, draw, right=0.4cm of ddim-1, label={below: $\textcolor{B}{\mathbf{x}_{0}^{(B)}}$}] (x-0) {
\includegraphics[scale=0.15]{figures/tex/pipeline_jpg/xb/1.jpg}
};

\draw[->] (ddim-1) -- (x-0);

\begin{pgfonlayer}{bbackground}
\node [fit=(x-copy)(unet)(n)(ddim)(c)(x-0)(x-name)(step-name), fill=aaddgg!10, label={right: \rotatebox{-90}{%Generated given condition 
$\textcolor{B}{\mathbf{c}^{(B)}}$}}] {}; 
\end{pgfonlayer}
\end{tikzpicture}
}
